FGLP: A Federated Fine-Grained Location Prediction System for Mobile Users

Fine-grained location prediction on smart phones can be used to improve app/system performance. Application scenarios include video quality adaptation as a function of the 5G network quality at predicted user locations, and augmented reality apps that speed up content rendering based on predicted user locations. Such use cases require prediction error in the same range as the GPS error, and no existing works on location prediction can achieve this level of accuracy. We present a system for fine-grained location prediction (FGLP) of mobile users, based on GPS traces collected on the phones. FGLP has two components: a federated learning framework and a prediction model. The framework runs on the phones of the users and also on a server that coordinates learning from all users in the system. FGLP represents the user location data as relative points in an abstract 2D space, which enables learning across different physical spaces. The model merges Bidirectional Long Short-Term Memory (BiLSTM) and Convolutional Neural Networks (CNN), where BiLSTM learns the speed and direction of the mobile users, and CNN learns information such as user movement preferences. FGLP uses federated learning to protect user privacy and reduce bandwidth consumption. Our experimental results, using a dataset with over 600,000 users, demonstrate that FGLP outperforms baseline models in terms of prediction accuracy. We also demonstrate that FGLP works well in conjunction with transfer learning, which enables model reusability. Finally, benchmark results on several types of Android phones demonstrate FGLP's feasibility in real life.

==> benchmark.tex <==
\subsection{Model Benchmarks on Smart Phones}
\label{sec:benchmark}
{\fontfamily{ptm}\selectfont
\subsubsection{Inference Performance}

\textbf{Implementation and Settings.}
The prototype model used so far was developed in TensorFlow. While TensorFlow and TensorFlow Lite training are not supported in Android, we can download the server-trained model on the phone to perform prediction. Since the TensorFlow model is heavier than versions developed in TensorFlow Lite or DL4J, the performance and resource consumption of such a model act as upper bounds for lighter model implementations.

We converted the server-trained model to a TensorFlow protocol buffer (pb) file, and the model takes 67MB on the phone. We developed a benchmark app on Android to load the model and perform predictions for a given input.  

The maximum memory usage is verified using the Android Profiler in Android Studio. The running time per prediction is calculated by averaging 100 predictions. After leaving the app running in background for 2 hours to perform predictions in a loop, the battery consumption is computed from the percentage of power usage measured by Battery Historian~\footnote{https://github.com/google/battery-historian}. The battery statistics are reset after switching the app to the background to make sure the app foreground usage is not included.

\textbf{Results.}
We test the model on three phones with different specs, as shown in Table~\ref{phone}. The results in Table~\ref{inference} demonstrate low resource consumption and good prediction latency. The maximum RAM usage of FGLP is less than 200MB. The Google Pixel 3XL, a mid-range phone in 2020, can make a prediction in 46.41ms, which is fast enough for all practical purposes. On the same phone, the battery consumption per prediction is 0.0238$\mu$Ah, and 129 million predictions can be executed with a full battery. With further optimization, such as model pruning and compression, the resource consumption can be even lower. These results demonstrate that the model can be deployed effectively in real life. 




\begin{table}[t!]
\centering
\caption{Smart phone specs }
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
Phone Model          
              & \shortstack{ Android\\ Version}
                 & \shortstack{ Battery Capacity\\ (mAh)}  & \shortstack{ CPU\\ (GHz)} & \shortstack{ RAM\\ (GB)}   \\ \hline
ZTE Blade V8 Pro                    & 6          & 2213   &   8x2.0  &   3        \\ \hline
Huawei Nexus 6P                  & 7                & 2986  & 4x1.55; 4x2.0   &   3 \\ \hline
Google Pixel 3XL              & 10                     & 3082  & 4x2.5; 4x1.6  &   4 \\ \hline
\end{tabular}}
\label{phone}
\end{table} 

\begin{table}[t!]
\centering
\caption{Inference resource consumption and latency}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
Phone Model          
                & \shortstack{ Maximum \\RAM \\Usage \\ (MB) } & \shortstack{ Running \\ Time per \\ Prediction\\(ms) }
                 & \shortstack{Battery \\ Consumption\\ per Prediction\\ ($\mu$Ah)}  & \shortstack{ Millions of \\Predictions \\for Full\\ Battery }   \\ \hline
ZTE Blade V8 Pro        &187  & 207.47                      & 1.87   & 1.18         \\ \hline
Huawei Nexus 6P         &192  & 79.68                        & 1.11  & 2.69   \\ \hline
% Google Pixel 3XL        &167  & 46.41                         & 0.0238  & 129.28   \\ \hline
Google Pixel 3XL        &167  & 46.41                         & 0.238  & 12.93   \\ \hline
\end{tabular}}
\label{inference}
\end{table} 

\subsubsection{Training Performance}

\textbf{Implementation and Settings.}
Since TensorFlow and TensorFlow Lite do not support on-device training currently, we implement FGLP in DL4J. The model takes 50MB in a zipped bin and json format. We develop a benchmark app on Android to load the initial model received from the server and perform one round of training from pre-processed data. We implement the training with Android native AsyncTask class, which will not be terminated by Android even when the app is idle. The same tools and methods as in the previous experiment are used to measure resource consumption.

The training time is recorded by training 200 samples for 20 epochs, which is the optimum scenario determined in Section~\ref{sec:federated}. Foreground training is done while leaving the screen on, and it uses the full single core capacity. It provides a lower bound for the training time. 
%Realistically, however, we expect training to be done in the background, either on battery or on charger.

As in real world, other apps or system processes may interfere with training. We take 10 measurements for each benchmark, and report the mean and standard deviation.

\textbf{Results.}
Table~\ref{training} shows the training time and the resource consumption on the phones. The results demonstrate that training is feasible in real-life, even without optimizing the models. The maximum RAM usage of FGLP is less than 753 MB, and current phones are equipped with sufficient RAM to handle it. We observe quite different training times among different phones. The foreground training time demonstrates the full computation capacity of a single core, and the most powerful phone, Pixel 3XL, has the shortest time. We do not report battery consumption on foreground, as the screen consumes a much larger amount of energy that training. 

The background training time on charger, which is the expected situation for FL training, is reasonable in practice. On two phones, the training time is similar with the foreground time; only one phone experiences a significantly higher training time. The explanation for the newer phone model performing worst is related to the newer Android version it uses (10 vs. 6 and 7 on the other two phones). According to Google, from Android 9, to ensure that system resources are given to the apps that need them the most, the system limits apps' access to device resources like the CPU or battery based on the user's usage patterns.

We also performed experiments for background training on battery. The results on the older phones are reasonable in terms of both training time and battery consumption. However, the training time on the new phone is not acceptable for the same reason discussed above. We also observe that the training time for foreground and background on charger varies much less than background training time on battery. This is because once the task goes to background, other apps or system processes are more likely to interfere with the training process over a longer period of time.

To conclude, the results show that FGLP with FL is feasible in practice. Typically, the model would not have to be trained more than once a day because it needs enough new data to participate in a new round of training. Our results show that all phones can perform this training in the background while charging in less than 15 min. 
%Performing background training on battery is possible, but it requires a solution to the new Android-imposed limitations on background tasks.

\begin{table}[t!]
\centering
\caption{Training resource consumption and latency}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Phone Model          
                & \shortstack{ Maximum \\RAM\\ Usage \\ (MB) } & \shortstack{ Foreground \\ Training \\ Time \\ Mean/SD \\(min) } & \shortstack{ Background \\ Training Time \\ on Charger \\ Mean/SD\\ (min) } & \shortstack{ Background \\Training Time \\ on Battery \\ Mean/SD \\(min) }
                 & \shortstack{Battery \\ Consumption \\ per\\ Round \\ (mAh)}  & \shortstack{ Number of \\Training \\ Rounds\\ for Full\\ Battery }   \\ \hline
ZTE Blade V8 Pro        &743  & 6.84/0.30   & 6.81/0.04   & 7.54/1.09    & 87.52   & 25         \\ \hline
Huawei Nexus 6P         &753  & 9.94/0.94   & 8.94/0.32   & 44.90/13.52     & 114.63  & 26   \\ \hline
Google Pixel 3XL        &592  & 2.65/0.34  & 14.34/0.10   & 375.49/126.57   & 15.16  & 203   \\ \hline
\end{tabular}}
\label{training}
\end{table} 
}

==> discussion.tex <==
\section{Discussion}
\label{sec:disc}
{\fontfamily{ptm}\selectfont
%This section discusses issues related to real-life deployment of FGLP and expands on the use cases presented so far.

%For a real-life deployment, an important question is who will maintain the FGLP server? We believe the server can be maintained by phone manufacturers or by companies that control the phone OSs. These companies have an incentive to improve the phone and app performance using location prediction on the phones.

% So far, all our use cases involved software running on the phones only. However, location prediction could also be used by Internet services accessed from the phones. An example is represented by enhanced location-based services (LBSs) that use predicted user locations instead of current user locations. Such an LBS could increase the revenue associated with location-based ads by delivering only relevant ads on the user's predicted path. The advantage of FGLP for such a use case is that users do not have to share location traces with enhanced LBSs, but just predictions computed on the phones.

% In FGLP, there is a trade-off between prediction accuracy and privacy. Specifically, the accuracy is higher when FGLP does not use FL. In such a case, the relative input data is submitted to the server, which performs training and prediction. The output of the prediction is an abstract grid-cell, which is sent back to the phone. The phone can translate this abstract grid-cell into a physical grid-cell. In addition to higher accuracy, this use of FGLP reduces the computation and battery power needed on phones when compared with FGLP using FL. Furthermore, without additional external information, the server cannot learn the physical location of the user because the server handles only relative data. 

% Nevertheless, more sophisticated location inference attacks are possible at the server if FL is not used. If the attacker learns one physical location in a sequence by physically observing the user, it is easy to determine the whole sequence. Then, based on the sequence, the attacker may infer the user identity~\cite{gruteser2005anonymity,xu2009feeling} and link it to the visited locations. 

The FGLP model can also be used for service providers that have access to user location traces. Two examples are cellular network operators or map services that provide turn-by-turn routing to destinations. While the abstract representation of data in FGLP is not necessary for privacy protection in this use case because the providers already know the physical locations of the users, FGLP is expected to lead to better prediction performance than models using physical data. This is because its abstract data representation eliminates the training bias introduced by physical location data.

% Network operators can use accurate location prediction in 5G networks at every time scale and across all layers of the protocol stack \cite{6924849}. Minute-scale location prediction can benefit many applications, including proactive caching, load balancing, scheduling, synchronization, topology, power control, resource allocation, and handover~\cite{6924849}. At the physical layer, by tracking and predicting the change in mobile user movements, the weights of antenna elements can be dynamically optimized for best signal coverage while incurring minimum interference from other users. Furthermore, our model can easily be configured for different spatial and temporal scales, which may allow providers to use differently configured models for different cities or different days of the week.

%Premium services provided by network operators can take advantage of accurate location predictions to free up resources at crowded target locations ahead of time to ensure the best network performance for premium customers when they reach these destinations. The Open Radio Access Networks (O-RAN) ~\cite{oran2020techreport} propose to optimize RAN resources to provide better network connectivity to smart phone users. One such optimization can be to intelligently take advantage of accurate location prediction of users. 
}
